Wave Physics-informed Matrix Factorizations

With the recent success of representation learning methods, which includes deep learning as a special case, there has been considerable interest in developing techniques that incorporate known physical constraints into the learned representation. As one example, in many applications that involve a signal propagating through physical media (e.g., optics, acoustics, fluid dynamics, etc), it is known that the dynamics of the signal must satisfy constraints imposed by the wave equation. Here we propose a matrix factorization technique that decomposes such signals into a sum of components, where each component is regularized to ensure that it {nearly} satisfies wave equation constraints. Although our proposed formulation is non-convex, we prove that our model can be efficiently solved to global optimality. Through this line of work we establish theoretical connections between wave-informed learning and filtering theory in signal processing. We further demonstrate the application of this work on modal analysis problems commonly arising in structural diagnostics and prognostics.

==> letter_for_reviewers.tex <==
% !TeX root = bare_jrnl.tex

\newpage

\onecolumn

\setcounter{page}{1}

\section*{Letter to the Reviewer -- Response to the Decision Letter}

We would like to thank the editor and anonymous reviewers for their valuable time in reviewing our manuscript. We value each suggestion from the reviewers and have tried to incorporate/answer as many questions/suggestions as possible within the revised manuscript. We address the comments of the editor and reviewers below.

\subsection*{Associate Editor}

\textcolor{blue}{\textbf{Comment:} Based on the enclosed set of reviews, your manuscript requires a MAJOR REVISION (RQ). As you will see, all three reviewers acknowledge the novelty and interest of your problem. On the other hand, they say that the algorithm and its analysis essentially follow previous work. I think this may not be a redhibitory issue (solving a new problem with a somewhat standard algorithm is already an interesting contribution), but, as one of the reviewers asks, it would be good if you could modify your article so as to better highlight what is new and what is a adaptation of similar results from the literature.}

\textbf{Response:} Thank you for the positive response and suggestions! In light of your suggestions to better highlight what is new and what is an adaptation of similar results from the literature, we have modified  the contributions subsection (\ref{subsection:contributions}) to mention (in order of precedence) the three major contributions of this work:

\begin{quote}
``In this work we make the following contributions. We \emph{first} introduce a \textit{\textbf {wave-informed matrix factorization model}}, which ensures that the recovered components minimize wave equation constraints, allowing for direct interpretability of the factors based on assumed physics.''

\ldots

``\emph{Second}, although our resulting formulation requires solving a \emph{non-convex} optimization problem, we identify its form amenable to be provably solved to global optimality \cite{haeffele2019structured}. This differs from prior wave-physics informed dictionary learning \cite{Tetali2019}, which provides no such guarantees.''

\ldots

``\emph{Third}, unlike physics-informed neural networks, we show that our wave physics-informed matrix factorization has a satisfying interpretation as an optimal filter problem. Specifically, we show that our  optimization algorithm based on \cite{haeffele2019structured} reveals a solution is that of an optimal bank of 1st-order Butterworth filters. This interpretability enables confidence in the algorithm and intelligent selection of  hyper-parameters.''


\end{quote}
In addition, we explain the novelty in this work, arising from the three major contributions:
\begin{quote}
``In summary, this work's novel contributions are in demonstrating the first framework for matrix factorization that is constrained solely on the wave equation. Unlike wave-informed dictionary learning \cite{Tetali2019}, we show this algorithm is both highly interpretable from a signal processing perspective and satisfies global optimality conditions based on results the literature \cite{haeffele2019structured}. Finally, we evaluate the effectiveness of the algorithm in four scenarios -- homogeneous vibrations, non-homogeneous vibrations, travelling plane waves, and segmented vibrations. We show that this framework outperforms most other methods used the literature for wave mode decomposition, particularly in the presence of high noise and segmented, spatially varying wave behavior.''
\end{quote}
We also briefly describe in the beginning of \ref{others} what each subsection in \ref{others} contains. In doing so, we also emphasize which subsections are novel and which are extensions of existing work.

\begin{quote}
``{In subsection} \ref{subsection:problem_formulation}, {we introduce our objective function. This subsection can be seen as an extension of the previously proposed wave-informed dictionary learning framework to a matrix factorization framework. In} \ref{section:model}, {we go over a few ideas from the optimization literature that are useful to solve the formulated problem. In} \ref{subsection:polar} {and} \ref{subsection:WIMF}, {we describe the main portions of the wave-physics informed matrix factorization algorithm.} {In} \ref{sec:sig_procc}, {we describe an interesting connection of this framework to signal processing. We emphasize that the novel parts of this work is in subsections} \ref{subsection:polar} {and} \ref{sec:sig_procc}. The work optimization discussions in \ref{section:model} {are specific cases of previous work and are shown for the benefit of the reader, particularly those in wave physics who may not be familiar with the optimization literature.}''
\end{quote}
Beyond this point, as we also note in the paper and as is detailed in \cite{haeffele2019structured}, the main optimization challenge from a computational standpoint is whether or not the polar problem can be solved.  In particular, in the paper we note:

\begin{quote}
``Despite the fact that \cite{haeffele2019structured} gives a meta-algorithm is guaranteed to solve \eqref{eq:gen_obj} to global optimality, one needs to solve the polar problem in \eqref{eq:polar_def} to both verify global optimality and escape non-optimal stationary points, which is itself another optimization problem. This presents a potentially significant computational challenge in practice, as for many choices of regularization function, solving the polar problem is NP-hard \cite{bach2013convex}. For example, if the regularization on the matrix columns is simply the sum of the $\ell_2$ norms of the columns, then the polar problem is easily solved as a maximum eigenvalue problem, but if we either replace one of the $\ell_2$ norms by the $\ell_\infty$ norm, the problem becomes NP-hard \cite{bach2013convex}.  Fortunately, however, in the next section we show that the polar problem that results from our wave-informed factorization model is tractable and leads to polynomial time global optimality.''
\end{quote}
Based on this fact, we note that the main contribution from an optimization standpoint is a proof and computationally efficient algorithm to solve the polar problem associated with our particular choice of wave-informed regularizer.  Finding a regularizer that both captures desired structure in the problem while still resulting in a polar problem that can be feasibly computed is very non-trivial and the a contribution with regards to optimization. We further emphasize at the start of \ref{subsection:problem_formulation} that these concepts that are new and distinguish them from already existing concepts:
\begin{quote}
``{The problem formulation described in this section is inspired from the wave-physics regularizer proposed in} \cite{Tetali2019}. {In this work, we additionally justify the wave-physics informed problem formulation in} \cite{Tetali2019} {as a naturally arising idea from the theory of solutions of partial differential equations.}''
\end{quote}


\newpage
\subsection*{Reviewer 1}

\textcolor{blue}{\textbf{Comment 0:}  Overall, this work looks good. The idea of studying wave physics-informed matrix factorization seems novel and reasonable. The authors also provide theoretical guarantees for the proposed algorithm and compare the performances among different algorithms. However, there remain some shortcomings, which are listed below.}

\textbf{Response 0:} We thank the reviewer for their acknowledgment of the novelty of our approach and noting the overall positive aspects of our work.  In regards to the reviewer's specific questions and concerns we note the following revisions/answers.
\vspace{1em}
% \begin{enumerate}
% \setlength{\itemsep}{12pt}
% \setlength{\parskip}{6pt}

\textcolor{blue}{\textbf{Comment 1:}  I feel it would be better to have a related work section to systematically introduce the previous work and how they relate to this work. So far, it is unclear to me which part is new and which part is adopted of earlier works.} 

\textbf{Response 1:}  Thank you for your suggestion to improve our manuscript.  We have restructured the papers introduction to include ``Related Works'' and ``Contributions'' sections to make it clear what is new and from the literature.  In addition, we have clarified the novelty of this work within the ``Contributions'' section. Please see our response to the associate editor for this information. 


\vspace{1em}
\textcolor{blue}{\textbf{Comment 2:} 
``Polynomial running time.'' In Corollary 1, the authors claim that their algorithm (Algorithm 1) has a polynomial running time. However, throughout the work, I cannot find the iteration complexity. Based on my understanding, the authors only guarantee that the running time for the polar problem is polynomially-solvable. However, it is totally possible that the total running time is exponentially slow. I conjecture that we can show that the objective value can decrease rapidly, and the algorithm is indeed polynomially-solvable. I suggest clearly writing down the convergence rate in terms of dimension and other parameters instead of claiming that it can be solved in polynomial time.  
}

\textbf{Response 2:}  It would be possible to provide a formal result as the reviewer suggests, but in our opinion, it was not particularly worthwhile to do so in this paper due to the fact that Algorithm 1 uses a mix of optimization approaches (i.e, first perform alternating block coordinate gradient descent to reach a stationary point, then apply a Frank-Wolfe/conjugate-gradient step with the polar solution to escape any poor minima, then return to block coordinate gradient descent), each of which has been shown in prior work to make provable sufficient progress in each iteration to efficiently converge to the solution.  For example, the authors of \cite{xu2013block} prove that the block coordinate gradient descent portion of the algorithm will converge to a stationary point at a rate of $\mathcal{O}(1/t)$ (with $t$ being the number of iterations), which can be improved to $\mathcal{O}(1/t^2)$ with Nesterov acceleration.  Likewise, the authors of \cite{bach2013convex} show that repeated application of a Frank-Wolfe/conjugate-gradient step (i.e., when we escape poor stationary points by solving the polar problem) will converge to a global minimizer with a linear convergence rate.  Formally proving an overall convergence rate of Algorithm 1 would be possible by combining arguments from this prior work, but in our opinion this would be a relatively minor contribution and substantially increase the length of the manuscript/supplement while also somewhat shifting the focus of the paper to pure optimization and distracting from the modeling and signal processing aspects or our current paper.  

Moreover, Algorithm 1 is simply one choice of algorithm to optimize the overall model and many comparable results could be proven with alternative algorithms (i.e., adding Nesterov acceleration, momentum, etc.). The ability to verify global optimality and escape non-optimal stationary points, provided by the ability to solve the polar problem, enables many potential variants for optimization and hence why we focus our formal results on detailing the polar problem solution, which is the key contribution of our work in regards to optimization and ensuring global optimality. % \hl{ Should we then soften the language on polynomial running time? We could also demonstrate it empirically. --Joel } \hl{I don't think we need to soften the language since it will run in polynomial time, but I do think it might be good to remove the `formal' corollary about polynomial run-time time since we're not actually showing the full proof of polynomial time (which as I write above we could do, but it'd be pretty tedious and turn this into more of a pure optimization paper) -- Ben}.  \qquad \hl{Sounds good. I have commented out the corrollary. --Joel }


Nevertheless, we acknowledge and appreciate the reviewer's comment, as we also debated how to best approach these issues in our initial writing.  In our revised manuscript, we have added some of our above discussion on the previously given rates of convergence for the various pieces of Algorithm 1, how Algorithm 1 is simply one potential choice of optimization algorithm, and how the polar problem solutions enables many potential alternative strategies to achieve global optimality. This additional discussion can be found at the end of section \ref{subsection:WIMF}, where we have added the following text:

\begin{quote}
``Taken together, our proposed algorithm results in a polynomial-time algorithm for solving our main objective \eqref{eq:main_obj}. We do not give a formal result as the algorithm given in Algorithm \ref{alg:meta} is simply one choice of optimization algorithm which is possible due to the polynomial time solution for the polar problem that we give in Theorem \ref{thm:polar} and much of the overall convergence of the algorithm is known from prior work, provided the polar problem can be solved.  For example, the authors of \cite{xu2013block} prove that the block coordinate gradient descent portion of the algorithm will converge to a stationary point at a rate of $\mathcal{O}(1/t)$ (with $t$ being the number of iterations), which can be improved to $\mathcal{O}(1/t^2)$ with Nesterov acceleration.  Likewise, the authors of \cite{bach2013convex} show that repeated application of a Frank-Wolfe/conjugate-gradient step (i.e., when we escape poor stationary points by solving the polar problem) will converge to a global minimizer with a linear convergence rate.  From this it is straight-forward to combine these arguments to give an overall guarantee of convergence, but we do not do so here to limit the scope and length of the manuscript.''
\end{quote}


%\hl{I could not find this discussion. I may have found the them, but am unsure... --Joel } \hl{Haven't added yet, but basically merging the discussion in this response with our `proof' of the corollary about overall polynomial runtime. --Ben}

\vspace{1em}

\textcolor{blue}{\textbf{Comment 3:}  
''Lipschitz constant $L_k$ in equation 19, the authors provide the Lipschitz constant for the line-search subproblem. Here, my question is that this constant depends on the norm of $Y-DX$, which will vary during the optimization process. Hence, we need to show that $\|Y-DX\|$ won't blow up in the training process. However, I think this won't be too difficult since the objective value should decrease over the time. But, this issue should be explicitly mentioned in the main text.
}

\textbf{Response 3:} It is straight-forward to see the residual term will not explode, provided gradient descent does not diverge when attempting to find a first-order stationary point (which will be the case for an appropriately small choice of step-size).  To see this, consider a very simplified problem, where we hold the directions of $\D$ and $\X$ fixed in \eqref{eq:main_obj} and we simply optimize over a scalar multiplication of $\X \rightarrow \alpha \X$.  I.e., we want to solve:
%
\begin{equation}
\min_{\alpha} \tfrac{1}{2} \| \Y - \D (\alpha \X)^\top \|_F^2 + \tfrac{\lambda}{2} \| (\alpha \X) \|_F^2 + \tfrac{\lambda}{2} \sum_{i=1}^N \d_i^\top \A(k_i) \d_i
\end{equation}
%
It is easily shown that the optimal value for $\alpha$ in this case (assuming we are not in the trivial case where $\D$ or $\X$ are all-zeros) is given as:
%
\begin{equation}
\alpha^* = \frac{\langle \D \X^\top , \Y \rangle} {\| \D \X^\top \|_F^2 + \lambda \| \X \|_F^2}
\end{equation} 
%
Evaluating the residual for this optimal scaling of $\X$ gives:
%
\begin{equation}
\tfrac{1}{2} \|\Y - \D (\alpha^* \X)^\top \|_F^2 = \tfrac{1}{2}\||\Y\|_F^2 + \frac{ ( \langle \Y, \D \X^\top \rangle )^2} {\| \D \X^\top \|_F^2 + \lambda \|\X\|_F^2}  \left( \frac{ \|\D \X^\top \|_F^2} {\| \D \X^\top \|_F^2 + \lambda \| \X\|_F^2} - 1 \right) \leq \tfrac{1}{2} \| \Y \|_F^2
\end{equation}
%
where the final inequality can be seen by noting the term in the final parenthesis is always non-positive and the leading coefficient is non-negative.  Note that any first-order stationary point will be at an optimal scaling of $\alpha$ since otherwise we can improve the objective by simply scaling $\X$, which would imply we are not at a first order stationary point.  As a result, we have that the residual term when we evaluate it in Algorithm 1 will always be bounded at least by $\tfrac{1}{2} \|\Y\|_F^2$ (and much tighter bounds could likely be derived if one was interested).   We have added the above discussion to the Supplemental Material after Corollary \ref{cor:line_search}.

\vspace{1em}

\textcolor{blue}{\textbf{Comment 4:} 
``Issue in the pseudocode in Algorithm 1''. In the first iteration in the while loop, tilde D, and X are not defined. I think they should also be initialized the same as $\D$, $\X$.}
 
\textbf{Response 4:} Thank you for noticing this! We have addressed this in the algorithm block by adding:
\begin{quote}
    Initialize $ \left( \tilde{\mathbf{D}}, \tilde{\mathbf{X}}, \tilde{\mathbf{k}} \right) \leftarrow \left( \mathbf{D}_{init}, \mathbf{X}_{init}, \mathbf{k}_{init} \right)$
\end{quote}

\vspace{1em}

\textcolor{blue}{\textbf{Comment 5:}  
5. "Optimal value of tau in equation 25". How to guarantee the term in the square root is nonnegative?
}

\textbf{Response 5:} This is already guaranteed due to the fact that $(\d^*,\x^*)$ is an optimal solution to the polar problem.  If the term in the square root was not strictly positive, then from the definition of $\Omega^\circ$ this is equivalent to the condition that $\Omega^\circ (\tfrac{1}{\lambda} (\Y - \D \X^\top)) \leq 1$, which would have triggered the stopping condition in Algorithm 1 (also see the discussion above~\eqref{eqn: updates}).
\vspace{1em}
    
\textcolor{blue}{\textbf{Comment 6:}  
"The argument below equation 43". How can you take the maximum of k for a function d'Zx that does not contain k? If this argument is wrong, then the proof of Theorem 1 might be wrong.
} 

\textbf{Response 6:} Note that the constraint in \eqref{eqn:polar_descrip} is dependent on $k$. To clarify, the constraint is $\| \x \|^2_2 \leq 1, \|\d\|^2_2 + \gamma \min_{k} \| \L \d + k^2 \d \|^2_2 \leq 1$, which has $k$ in it, thus, making the optimization problem (and the optimal $\mathbf{d}$ and $\mathbf{x}$) dependent on $k$. 

\vspace{1em}


\textcolor{blue}{\textbf{Comment 7:}  
"Small typos." There exist several small typos. For example, in the right hand of line 11, theta should be bar theta; Line 33 left-hand side, double proven; In the right-hand side of line 59, miss a period.
} 

\textbf{Response 7:} 
Thank you spotting these typos. We have corrected added the bar to $\theta$ and included the missing period. However, we were not entirely sure what the reviewer meant by ``double proven,'' so there have been no changes based on that. 


\newpage
\subsection*{Reviewer 2}

\textcolor{blue}{\textbf{Comment 0:}  
This paper considers the problem of factoring a data matirx
Y into the form $Y = DX^T$, where the matrix factors D, X are subject
to physical constraints. To solve this problem the authors formulate
this factorization problem as a minimization problem over D, X and
adds an additional regularization term to enforce the physical
constraints (based on the discretization of the wave equation).}

\textcolor{blue}{
I think the results of the paper, particularly the numerical section
and the connection to the butterworth filter is interesting.
}

\textbf{Response 0:} We thank the reviewer for their positive comment! Identifying the value of the results and its signal processing connection with our physics-informed factorization are two of the main objectives of this paper. 
\vspace{1em}

\textcolor{blue}{\textbf{Comment 1:}}  
\textcolor{blue}{
My main concern regarding novelty is with the the proposed algorithm.
The authors essentially propose a first-order alternate descent
algorithm, as is common for these type of problems (such as
dictionary learning). If such a first-order algorithm is stuck at,
one can check this by a simple condition proposed in [38] and proceed
to augment the current point by appending a new column. The new
column can be formulated as the solution to a polar problem (16).
}

\textcolor{blue}{
This algorithmic framework, and its proof of convergence, was almost
completely fleshed out already in [38]. The only new analysis in this
paper pertains to the observation that the polar problem (16) can be
solved efficiently within the context of this paper.
}

\textcolor{blue}{
Therefore, while I believe the problem formulation itself is
interesting, from an algorithmic perspective, this paper has limited
novelty, because it simply adapts a previous well-studied algorithm
to the specific situation in this paper.
}

\textbf{Response 1:}
 %We agree with reviewer 2 that the optimization algorithm is not the most novel part of the article, and was mostly described for the benefit of the readers to maintain a continuous flow and completeness. We apologize for this confusion. 
Please see our response to the Associate Editor, where we address and clarify the novel contributions of this work in regard to optimization and guaranteeing global optimality.

In addition, we also share reviewer 2's (as well as the other two reviewers') interest in the application and signal processing interpretation of physics-informed framework and algorithm, which is a \textbf{unique fundamental theme} that we introduce through this work in addition to the wave-informed matrix factorization framework. Our new text detailed in the response to the Associate Editor also further clarifies these contributions. In addition, we also add to the end of subsection \ref{sec:sig_procc}:
\begin{quote}
``We would like to emphasize that this work introduces a unique theme within the works of scientific machine learning. Through means of wave-informed learning, we obtain a new method to mathematically derive the well-known \emph{digital Butterworth filter}.''
\end{quote} 


%\hl{We should also point to the comments to the Associate editor here --- joel }

%{This quote is different than what's in the paper... Which do we use? --Joel}


%We also share reviewer 2's interest in the numerical simulations and acknowledge them for their appreciation.

\newpage
\subsection*{Reviewer 3}

\textcolor{blue}{\textbf{Comment:}  
The manuscript "Wave Physics-Informed Matrix Factorizations" presents a matrix factorization method for decomposing signals into components that satisfy the wave equation, as opposed to purely data-driven methods such as PCA, which are not constrained by physical knowledge. The proposed approach also differs from more constrained approaches that parameterize physics-respecting wave-like factors.
}

\textcolor{blue}{
The method consists of a non-convex optimization problem for the factors with a physics-informed regularization term that penalizes deviations of the residual of the Helmholtz equation applied to the factors. The authors show that even though this optimization problem is non-convex, there exist an algorithm for obtaining a global minimum if the minimization over the wavenumber is understood to be incorporated into the regularizer, and formulate such an algorithm. The authors compare the method against state-of-the-art approaches such as ICA, DMD, and EMD, among others. They find their method to be best or second-best for most numerical experiments considered.
}

\textcolor{blue}{
I believe this manuscript represents a valuable contribution to the state-of-the-art in
physics-informed scientific machine learning and warrants publication. My only comment is that the authors should be more upfront about the fact that the factorization doesn't exactly satisfy the wave equation because the physics-informed penalty is introduced as a "soft" constrain, leading to an unconstrained minimization problem. Specifically, the authors in the abstract and introduction make statements such as that their construction "ensures" that the factorization "satisfies wave equation constraints", or that they "ensure" that the factorization "minimize[s] wave equation constraints". This is not accurate and the authors point it out in Section IV.F. This is not a bad thing per se, and is a feature of PINNs and similar methods that they cite, but it requires some
care because the results of these physics-deviation-penalizing approaches are almost but not exactly physics respecting.
}


\textbf{Response:} Thank you for the positive response about the valuable contribution of the manuscript to physics-informed scientific machine learning! We would also like to thank reviewer 3 for pointing out the misleading wording in the abstract and section \ref{others}. In the abstract, instead of saying 
\begin{quote}
``... each component is regularized to ensure that it satisfies the wave equation constraints...''
\end{quote}
 we now say 
\begin{quote}
``each component is regularized to ensure that it \textbf{nearly} satisfies the wave equation constraints.''
\end{quote}


In \ref{others}, we change 
\begin{quote}
``where one of the matrices will be constrained to satisfy the wave equation constraints''
\end{quote} 
to 
\begin{quote}
``where one of the matrices will be \textbf{softly} constrained to \textbf{nearly} satisfy the wave equation constraints'' 
\end{quote}

==> reviews.tex <==

\newpage

\onecolumn

\section{Reviews}

Based on the enclosed set of reviews, your manuscript requires a MAJOR REVISION (RQ). As you will see, all three reviewers acknowledge the novelty and interest of your problem. On the other hand, they say that the algorithm and its analysis essentially follow previous work. I think this may not be a redhibitory issue (solving a new problem with a somewhat standard algorithm is already an interesting contribution), but, as one of the reviewers asks, it would be good if you could modify your article so as to better highlight what is new and what is an adaptation of similar results from the literature.


\subsection{Reviewer 1}

\textbf{Recommendation:} RQ - Review Again After Major Changes.

Overall, this work looks good. The idea of studying wave physics-informed matrix factorization seems novel and reasonable. The authors also provide theoretical guarantees for the proposed algorithm and compare the performances among different algorithms. However, there remain some shortcomings, which are listed below.

\begin{enumerate}
    \item I feel it would be better to have a related work section to systematically introduce the previous work and how they relate to this work. So far, it is unclear to me which part is new and which part is adopted of earlier works.
    \item ``\emph{Polynomial running time}'' In Corollary 1, the authors claim that their algorithm (Algorithm 1) has a polynomial running time. However, throughout the work, I cannot find the iteration complexity. Based on my understanding, the authors only guarantee that the running time for the polar problem is polynomially-solvable. However, it is totally possible that the total running time is exponentially slow. I conjecture that we can show that the objective value can decrease rapidly, and the algorithm is indeed polynomially-solvable. I suggest clearly writing down the convergence rate in terms of dimension and other parameters instead of claiming that it can be solved in polynomial time.
    \item ``Lipschitz constant $L_k$''. In equation 19, the authors provide the Lipschitz constant for the line-search subproblem. Here, my question is that this constant depends on the norm of $\Y-\D\X^{\top}$, which will vary during the optimization process. Hence, we need to show that $\|\Y-\D \X^{\top}\|$ won't blow up in the training process. However, I think this won't be too difficult since the objective value should decrease over the time. But, this issue should be explicitly mentioned in the main text.
    \item ``Issue in the pseudocode in Algorithm 1''. In the first iteration in the while loop, tilde D, and X are not defined. I think they should also be initialized the same as $\D$, $\X$.
    \item  ``Optimal value of $\tau$ in equation 25''. How to guarantee the term in the square root is nonnegative?
    \item ``The argument below equation 43''. How can you take the maximum of k for a function $\d^{\top}\Z\x$ that does not contain $k$? If this argument is wrong, then the proof of Theorem 1 might be wrong.
    \item ``Small typos''. There exist several small typos. For example, in the right hand of line 11, theta should be bar theta; Line 33 left-hand side, double proven; In the right-hand side of line 59, miss a period.
\end{enumerate}

\emph{Additional questions}:
\begin{enumerate}
    \item Is the topic appropriate for publication in these transactions?: Adequate Match

\item Is the paper technically sound?: Yes

\item How would you rate the technical novelty of the paper?: Novel Enough for Publication

Explain: The idea of "Wave Physics-Informed Matrix Factorization" is novel. On the other hand, this idea seems to be quite natural.

\item Is the contribution significant?: Moderately Significant

\item Is the coverage of the topic sufficiently comprehensive and balanced?: Treatment somewhat unbalanced, but not seriously so

\item Rate the Bibliography: Unsatisfactory

\item How would you rate the overall organization of the paper?: Satisfactory

\item Are the title and abstract satisfactory?: Yes

\item Is the length of the paper appropriate? If not, recommend what should be added or eliminated.: Yes


\item Are symbols, terms, and concepts adequately defined?: Not always

\item How do you rate the English usage?: Satisfactory


\end{enumerate}

\subsection{Reviewer 2}

\textbf{Recommendation:} R - Reject.

\emph{Additonal Questions}

\begin{enumerate}
    \item Is the topic appropriate for publication in these transactions?: Excellent Match

\item Is the paper technically sound?: Yes

\item How would you rate the technical novelty of the paper?: Not Novel

Explain: This paper considers the problem of factoring a data matirx Y into the form $\Y = \D \X^{\top}$, where the matrix factors $\D$, $\X$ are subject to physical constraints. To solve this problem the authors formulate this factorization problem as a minimization problem over $\D$, $\X$ and adds an additional regularization term to enforce the physical constraints (based on the discretization of the wave equation).

I think the results of the paper, particularly the numerical section and the connection to the butterworth filter is interesting.

My main concern regarding novelty is with the the proposed algorithm. The authors essentially propose a first-order alternate descent algorithm, as is common for these type of problems (such as dictionary learning). If such a first-order algorithm is stuck at, one can check this by a simple condition proposed in [38] and proceed to augment the current point by appending a new column. The new column can be formulated as the solution to a polar problem (16).

This algorithmic framework, and its proof of convergence, was almost completely fleshed out already in [38]. The only new analysis in this paper pertains to the observation that the polar problem (16) can be solved efficiently within the context of this paper.

Therefore, while I believe the problem formulation itself is interesting, from an algorithmic perspective, this paper has limited novelty, because it simply adapts a previous well-studied algorithm to the specific situation in this paper.

\item Is the contribution significant?: Moderately Significant

\item Is the coverage of the topic sufficiently comprehensive and balanced?: Yes

\item Rate the Bibliography: Satisfactory

\item How would you rate the overall organization of the paper?: Satisfactory

\item Are the title and abstract satisfactory?: Yes

\item Is the length of the paper appropriate? If not, recommend what should be added or eliminated.: Yes


\item Are symbols, terms, and concepts adequately defined?: Yes

\item How do you rate the English usage?: Satisfactory


\end{enumerate}


\subsection{Reviewer 3}


\textbf{Recommendation:} AQ - Publish With Minor, Required Changes


The manuscript "Wave Physics-Informed Matrix Factorizations" presents a matrix factorization method for decomposing signals into components that satisfy the wave equation, as opposed to purely data-driven methods such as PCA, which are not constrained by physical knowledge. The proposed approach also differs from more constrained approaches that parameterize physics-respecting wave-like factors.

The method consists of a non-convex optimization problem for the factors with a physics-informed regularization term that penalizes deviations of the residual of the Helmholtz equation applied to the factors. The authors show that even though this optimization problem is non-convex, there exist an algorithm for obtaining a global minimum if the minimization over the wavenumber is understood to be incorporated into the regularizer, and formulate such an algorithm. The authors compare the method against state-of-the-art approaches such as ICA, DMD, and EMD, among others. They find their method to be best or second-best for most numerical experiments considered.

I believe this manuscript represents a valuable contribution to the state-of-the-art in
physics-informed scientific machine learning and warrants publication. My only comment is that the authors should be more upfront about the fact that the factorization doesn't exactly satisfy the wave equation because the physics-informed penalty is introduced as a "soft" constrain, leading to an unconstrained minimization problem. Specifically, the authors in the abstract and introduction make statements such as that their construction "ensures" that the factorization "satisfies wave equation constraints", or that they "ensure" that the factorization "minimize[s] wave equation constraints". This is not accurate and the authors point it out in Section IV.F. This is not a bad thing per se, and is a feature of PINNs and similar methods that they cite, but it requires some
care because the results of these physics-deviation-penalizing approaches are almost but not exactly physics respecting.

\begin{enumerate}
    \item  Is the topic appropriate for publication in these transactions?: Adequate Match

\item Is the paper technically sound?: Yes

\item How would you rate the technical novelty of the paper?: Novel Enough for Publication

Explain: The manuscript "Wave Physics-Informed Matrix Factorizations" presents a matrix factorization method
for decomposing signals into components that satisfy the wave equation, as opposed to purely data-driven methods such as PCA, which are not constrained by physical knowledge. The proposed approach also differs from more constrained approaches that parameterize physics-respecting wave-like factors.

\item Is the contribution significant?: Significant

 \item Is the coverage of the topic sufficiently comprehensive and balanced?: Yes

\item Rate the Bibliography: Satisfactory

\item How would you rate the overall organization of the paper?: Satisfactory

\item Are the title and abstract satisfactory?: No

\item Is the length of the paper appropriate? If not, recommend what should be added or eliminated.: Yes


\item Are symbols, terms, and concepts adequately defined?: Yes

\item How do you rate the English usage?: Satisfactory

\end{enumerate}
